The Link Between Morphology and Structure of Brightest Cluster Galaxies: Automatic Identification of cDs

We study a large sample of 625 low-redshift brightest cluster galaxies (BCGs) and link their morphologies to their structural properties. We derive visual morphologies and find that ~57% of the BCGs are cD galaxies, ~13% are ellipticals, and ~21% belong to the intermediate classes mostly between E and cD. There is a continuous distribution in the properties of the BCG's envelopes, ranging from undetected (E class) to clearly detected (cD class), with intermediate classes (E/cD and cD/E) showing the increasing degrees of the envelope presence. A minority (~7%) of BCGs have disk morphologies, with spirals and S0s in similar proportions, and the rest (~2%) are mergers. After carefully fitting the galaxies light distributions by using one-component (Sersic) and two-component (Sersic+Exponential) models, we find a clear link between the BCGs morphologies and their structures and conclude that a combination of the best-fit parameters derived from the fits can be used to separate cD galaxies from non-cD BCGs. In particular, cDs and non-cDs show very different distributions in the $R_e$--$RFF$ plane, where $R_e$ is the effective radius and $RFF$ (the residual flux fraction) measures the proportion of the galaxy flux present in the residual images after subtracting the models. In general, cDs have larger $R_e$ and $RFF$ values than ellipticals. Therefore we find, in a statistically robust way, a boundary separating cD and non-cD BCGs in this parameter space. BCGs with cD morphology can be selected with reasonably high completeness (~75%) and low contamination (~20%). This automatic and objective technique can be applied to any current or future BCG sample with good quality images.

==> bib_in_latex <==
\begin{thebibliography}{40}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{{Barden} {et~al.}(2012){Barden}, {H{\"a}u{\ss}ler}, {Peng},
  {McIntosh}, \& {Guo}}]{Barden12}
{Barden} M., {H{\"a}u{\ss}ler} B., {Peng} C.~Y., {McIntosh} D.~H., {Guo} Y.,
  2012, \mnras, 422, 449

\bibitem[{{Bertin} \& {Arnouts}(1996)}]{BA96}
{Bertin} E., {Arnouts} S., 1996, \aaps, 117, 393

\bibitem[{{Bruce} {et~al.}(2012){Bruce}, {Dunlop}, {Cirasuolo}, {McLure},
  {Targett}, {Bell}, {Croton}, {Dekel}, {Faber}, {Ferguson}, {Grogin},
  {Kocevski}, {Koekemoer}, {Koo}, {Lai}, {Lotz}, {McGrath}, {Newman}, \& {van
  der Wel}}]{Bruce12}
{Bruce} V.~A., {Dunlop} J.~S., {Cirasuolo} M., {McLure} R.~J., {Targett} T.~A.,
  {Bell} E.~F., {Croton} D.~J., {Dekel} A., {Faber} S.~M., {Ferguson} H.~C.,
  {Grogin} N.~A., {Kocevski} D.~D., {Koekemoer} A.~M., {Koo} D.~C., {Lai} K.,
  {Lotz} J.~M., {McGrath} E.~J., {Newman} J.~A., {van der Wel} A., 2012,
  \mnras, 427, 1666

\bibitem[{{Caon} {et~al.}(1993){Caon}, {Capaccioli}, \& {D'Onofrio}}]{Caon93}
{Caon} N., {Capaccioli} M., {D'Onofrio} M., 1993, \mnras, 265, 1013

\bibitem[{{Conroy} {et~al.}(2007){Conroy}, {Wechsler}, \&
  {Kravtsov}}]{Conroy07}
{Conroy} C., {Wechsler} R.~H., {Kravtsov} A.~V., 2007, \apj, 668, 826

\bibitem[{{de Vaucouleurs}(1948)}]{deVaucl48}
{de Vaucouleurs} G., 1948, Annales d'Astrophysique, 11, 247

\bibitem[{{Donzelli} {et~al.}(2011){Donzelli}, {Muriel}, \&
  {Madrid}}]{Donzelli11}
{Donzelli} C.~J., {Muriel} H., {Madrid} J.~P., 2011, \apjs, 195, 15

\bibitem[{{Dressler}(1984)}]{Dressler84}
{Dressler} A., 1984, \apj, 281, 512

\bibitem[{{Fukugita} {et~al.}(1995){Fukugita}, {Shimasaku}, \&
  {Ichikawa}}]{fukugita95}
{Fukugita} M., {Shimasaku} K., {Ichikawa} T., 1995, \pasp, 107, 945

\bibitem[{{Gonzalez} {et~al.}(2005){Gonzalez}, {Zabludoff}, \&
  {Zaritsky}}]{Gonzalez05}
{Gonzalez} A.~H., {Zabludoff} A.~I., {Zaritsky} D., 2005, \apj, 618, 195

\bibitem[{{Graham} {et~al.}(2005){Graham}, {Driver}, {Petrosian}, {Conselice},
  {Bershady}, {Crawford}, \& {Goto}}]{Graham05}
{Graham} A.~W., {Driver} S.~P., {Petrosian} V., {Conselice} C.~J., {Bershady}
  M.~A., {Crawford} S.~M., {Goto} T., 2005, \aj, 130, 1535

\bibitem[{{Guo} {et~al.}(2009){Guo}, {McIntosh}, {Mo}, {Katz}, {van den Bosch},
  {Weinberg}, {Weinmann}, {Pasquali}, \& {Yang}}]{Guo09}
{Guo} Y., {McIntosh} D.~H., {Mo} H.~J., {Katz} N., {van den Bosch} F.~C.,
  {Weinberg} M., {Weinmann} S.~M., {Pasquali} A., {Yang} X., 2009, \mnras, 398,
  1129

\bibitem[{{H{\"a}u{\ss}ler} {et~al.}(2013){H{\"a}u{\ss}ler}, {Bamford}, {Vika},
  {Rojas}, {Barden}, {Kelvin}, {Alpaslan}, {Robotham}, {Driver}, {Baldry},
  {Brough}, {Hopkins}, {Liske}, {Nichol}, {Popescu}, \& {Tuffs}}]{Haubler13}
{H{\"a}u{\ss}ler} B., {Bamford} S.~P., {Vika} M., {Rojas} A.~L., {Barden} M.,
  {Kelvin} L.~S., {Alpaslan} M., {Robotham} A.~S.~G., {Driver} S.~P., {Baldry}
  I.~K., {Brough} S., {Hopkins} A.~M., {Liske} J., {Nichol} R.~C., {Popescu}
  C.~C., {Tuffs} R.~J., 2013, \mnras, 430, 330

\bibitem[{{H{\"a}ussler} {et~al.}(2007){H{\"a}ussler}, {McIntosh}, {Barden},
  {Bell}, {Rix}, {Borch}, {Beckwith}, {Caldwell}, {Heymans}, {Jahnke}, {Jogee},
  {Koposov}, {Meisenheimer}, {S{\'a}nchez}, {Somerville}, {Wisotzki}, \&
  {Wolf}}]{Haubler07}
{H{\"a}ussler} B., {McIntosh} D.~H., {Barden} M., {Bell} E.~F., {Rix} H.-W.,
  {Borch} A., {Beckwith} S.~V.~W., {Caldwell} J.~A.~R., {Heymans} C., {Jahnke}
  K., {Jogee} S., {Koposov} S.~E., {Meisenheimer} K., {S{\'a}nchez} S.~F.,
  {Somerville} R.~S., {Wisotzki} L., {Wolf} C., 2007, \apjs, 172, 615

\bibitem[{{Hopkins} {et~al.}(2009){Hopkins}, {Cox}, {Dutta}, {Hernquist},
  {Kormendy}, \& {Lauer}}]{Hopkins09}
{Hopkins} P.~F., {Cox} T.~J., {Dutta} S.~N., {Hernquist} L., {Kormendy} J.,
  {Lauer} T.~R., 2009, \apjs, 181, 135

\bibitem[{{Hoyos} {et~al.}(2011){Hoyos}, {den Brok}, {Verdoes Kleijn},
  {Carter}, {Balcells}, {Guzm{\'a}n}, {Peletier}, {Ferguson}, {Goudfrooij},
  {Graham}, {Hammer}, {Karick}, {Lucey}, {Matkovi{\'c}}, {Merritt}, {Mouhcine},
  \& {Valentijn}}]{Hoyos11}
{Hoyos} C., {den Brok} M., {Verdoes Kleijn} G., {Carter} D., {Balcells} M.,
  {Guzm{\'a}n} R., {Peletier} R., {Ferguson} H.~C., {Goudfrooij} P., {Graham}
  A.~W., {Hammer} D., {Karick} A.~M., {Lucey} J.~R., {Matkovi{\'c}} A.,
  {Merritt} D., {Mouhcine} M., {Valentijn} E., 2011, \mnras, 411, 2439

\bibitem[{{Huang} {et~al.}(2013){Huang}, {Ho}, {Peng}, {Li}, \&
  {Barth}}]{Huang13}
{Huang} S., {Ho} L.~C., {Peng} C.~Y., {Li} Z.-Y., {Barth} A.~J., 2013, \apjl,
  768, L28

\bibitem[{{Johansson} {et~al.}(2012){Johansson}, {Naab}, \&
  {Ostriker}}]{Johansson12}
{Johansson} P.~H., {Naab} T., {Ostriker} J.~P., 2012, \apj, 754, 115

\bibitem[{{Kron}(1980)}]{Kron80}
{Kron} R.~G., 1980, \apjs, 43, 305

\bibitem[{{Lauer} \& {Postman}(1992)}]{LP92}
{Lauer} T.~R., {Postman} M., 1992, \apjl, 400, L47

\bibitem[{{Liu} {et~al.}(2008){Liu}, {Xia}, {Mao}, {Wu}, \& {Deng}}]{Liu08}
{Liu} F.~S., {Xia} X.~Y., {Mao} S., {Wu} H., {Deng} Z.~G., 2008, \mnras, 385,
  23

\bibitem[{{Lugger}(1984)}]{Lugger84}
{Lugger} P.~M., 1984, \apj, 286, 106

\bibitem[{{Miller} {et~al.}(2005){Miller}, {Nichol}, {Reichart}, {Wechsler},
  {Evrard}, {Annis}, {McKay}, {Bahcall}, {Bernardi}, {Boehringer}, {Connolly},
  {Goto}, {Kniazev}, {Lamb}, {Postman}, {Schneider}, {Sheth}, \&
  {Voges}}]{Miller05}
{Miller} C.~J., {Nichol} R.~C., {Reichart} D., {Wechsler} R.~H., {Evrard}
  A.~E., {Annis} J., {McKay} T.~A., {Bahcall} N.~A., {Bernardi} M.,
  {Boehringer} H., {Connolly} A.~J., {Goto} T., {Kniazev} A., {Lamb} D.,
  {Postman} M., {Schneider} D.~P., {Sheth} R.~K., {Voges} W., 2005, \aj, 130,
  968

\bibitem[{{Oegerle} \& {Hill}(2001)}]{OH01}
{Oegerle} W.~R., {Hill} J.~M., 2001, \aj, 122, 2858

\bibitem[{{Oser} {et~al.}(2010){Oser}, {Ostriker}, {Naab}, {Johansson}, \&
  {Burkert}}]{Oser10}
{Oser} L., {Ostriker} J.~P., {Naab} T., {Johansson} P.~H., {Burkert} A., 2010,
  \apj, 725, 2312

\bibitem[{{Patel} {et~al.}(2006){Patel}, {Maddox}, {Pearce},
  {Arag{\'o}n-Salamanca}, \& {Conway}}]{Patel06}
{Patel} P., {Maddox} S., {Pearce} F.~R., {Arag{\'o}n-Salamanca} A., {Conway}
  E., 2006, \mnras, 370, 851

\bibitem[{{Peng} {et~al.}(2002){Peng}, {Ho}, {Impey}, \& {Rix}}]{Peng02}
{Peng} C.~Y., {Ho} L.~C., {Impey} C.~D., {Rix} H.-W., 2002, \aj, 124, 266

\bibitem[{{Peng} {et~al.}(2010){Peng}, {Ho}, {Impey}, \& {Rix}}]{Peng10}
---, 2010, \aj, 139, 2097

\bibitem[{{Petrosian}(1976)}]{Petrosian76}
{Petrosian} V., 1976, \apjl, 209, L1

\bibitem[{{Press} \& {Spergel}(1988)}]{Press88}
{Press} W.~H., {Spergel} D.~N., 1988, \apj, 325, 715

\bibitem[{{Schombert}(1986)}]{Schombert86}
{Schombert} J.~M., 1986, \apjs, 60, 603

\bibitem[{{Seigar} {et~al.}(2007){Seigar}, {Graham}, \& {Jerjen}}]{Seigar07}
{Seigar} M.~S., {Graham} A.~W., {Jerjen} H., 2007, \mnras, 378, 1575

\bibitem[{{S{\'e}rsic}(1963)}]{Sersic63}
{S{\'e}rsic} J.~L., 1963, Boletin de la Asociacion Argentina de Astronomia La
  Plata Argentina, 6, 41

\bibitem[{{Shen} {et~al.}(2003){Shen}, {Mo}, {White}, {Blanton}, {Kauffmann},
  {Voges}, {Brinkmann}, \& {Csabai}}]{Shen03}
{Shen} S., {Mo} H.~J., {White} S.~D.~M., {Blanton} M.~R., {Kauffmann} G.,
  {Voges} W., {Brinkmann} J., {Csabai} I., 2003, \mnras, 343, 978

\bibitem[{{Taylor-Mager} {et~al.}(2007){Taylor-Mager}, {Conselice},
  {Windhorst}, \& {Jansen}}]{TaylorMager07}
{Taylor-Mager} V.~A., {Conselice} C.~J., {Windhorst} R.~A., {Jansen} R.~A.,
  2007, \apj, 659, 162

\bibitem[{van Rijsbergen(1979)}]{vanRijsbergen79}
van Rijsbergen C.~J., 1979, Information Retrieval (2nd ed.).
  Butterworth-Heinemann, Newton, MA, USA

\bibitem[{{Vika} {et~al.}(2013){Vika}, {Bamford}, {H{\"a}u{\ss}ler}, {Rojas},
  {Borch}, \& {Nichol}}]{Vika13}
{Vika} M., {Bamford} S.~P., {H{\"a}u{\ss}ler} B., {Rojas} A.~L., {Borch} A.,
  {Nichol} R.~C., 2013, \mnras, 435, 623

\bibitem[{{von der Linden} {et~al.}(2007){von der Linden}, {Best}, {Kauffmann},
  \& {White}}]{Linden07}
{von der Linden} A., {Best} P.~N., {Kauffmann} G., {White} S.~D.~M., 2007,
  \mnras, 379, 867

\bibitem[{{Vulcani} {et~al.}(2014){Vulcani}, {Bamford}, {H{\"a}u{\ss}ler},
  {Vika}, {Rojas}, {Agius}, {Baldry}, {Bauer}, {Brown}, {Driver}, {Graham},
  {Kelvin}, {Liske}, {Loveday}, {Popescu}, {Robotham}, \& {Tuffs}}]{Vulcani14}
{Vulcani} B., {Bamford} S.~P., {H{\"a}u{\ss}ler} B., {Vika} M., {Rojas} A.,
  {Agius} N.~K., {Baldry} I., {Bauer} A.~E., {Brown} M.~J.~I., {Driver} S.,
  {Graham} A.~W., {Kelvin} L.~S., {Liske} J., {Loveday} J., {Popescu} C.~C.,
  {Robotham} A.~S.~G., {Tuffs} R.~J., 2014, ArXiv e-prints

\bibitem[{{Whiley} {et~al.}(2008){Whiley}, {Arag{\'o}n-Salamanca}, {De Lucia},
  {von der Linden}, {Bamford}, {Best}, {Bremer}, {Jablonka}, {Johnson},
  {Milvang-Jensen}, {Noll}, {Poggianti}, {Rudnick}, {Saglia}, {White}, \&
  {Zaritsky}}]{whiley08}
{Whiley} I.~M., {Arag{\'o}n-Salamanca} A., {De Lucia} G., {von der Linden} A.,
  {Bamford} S.~P., {Best} P., {Bremer} M.~N., {Jablonka} P., {Johnson} O.,
  {Milvang-Jensen} B., {Noll} S., {Poggianti} B.~M., {Rudnick} G., {Saglia} R.,
  {White} S., {Zaritsky} D., 2008, \mnras, 387, 1253

\bibitem[{{York} {et~al.}(2000){York}, {Adelman}, {Anderson}, {Anderson},
  {Annis}, {Bahcall}, {Bakken}, {Barkhouser}, {Bastian}, {Berman}, {Boroski},
  {Bracker}, {Briegel}, {Briggs}, {Brinkmann}, {Brunner}, {Burles}, {Carey},
  {Carr}, {Castander}, {Chen}, {Colestock}, {Connolly}, {Crocker}, {Csabai},
  {Czarapata}, {Davis}, {Doi}, {Dombeck}, {Eisenstein}, {Ellman}, {Elms},
  {Evans}, {Fan}, {Federwitz}, {Fiscelli}, {Friedman}, {Frieman}, {Fukugita},
  {Gillespie}, {Gunn}, {Gurbani}, {de Haas}, {Haldeman}, {Harris}, {Hayes},
  {Heckman}, {Hennessy}, {Hindsley}, {Holm}, {Holmgren}, {Huang}, {Hull},
  {Husby}, {Ichikawa}, {Ichikawa}, {Ivezi{\'c}}, {Kent}, {Kim}, {Kinney},
  {Klaene}, {Kleinman}, {Kleinman}, {Knapp}, {Korienek}, {Kron}, {Kunszt},
  {Lamb}, {Lee}, {Leger}, {Limmongkol}, {Lindenmeyer}, {Long}, {Loomis},
  {Loveday}, {Lucinio}, {Lupton}, {MacKinnon}, {Mannery}, {Mantsch}, {Margon},
  {McGehee}, {McKay}, {Meiksin}, {Merelli}, {Monet}, {Munn}, {Narayanan},
  {Nash}, {Neilsen}, {Neswold}, {Newberg}, {Nichol}, {Nicinski}, {Nonino},
  {Okada}, {Okamura}, {Ostriker}, {Owen}, {Pauls}, {Peoples}, {Peterson},
  {Petravick}, {Pier}, {Pope}, {Pordes}, {Prosapio}, {Rechenmacher}, {Quinn},
  {Richards}, {Richmond}, {Rivetta}, {Rockosi}, {Ruthmansdorfer}, {Sandford},
  {Schlegel}, {Schneider}, {Sekiguchi}, {Sergey}, {Shimasaku}, {Siegmund},
  {Smee}, {Smith}, {Snedden}, {Stone}, {Stoughton}, {Strauss}, {Stubbs},
  {SubbaRao}, {Szalay}, {Szapudi}, {Szokoly}, {Thakar}, {Tremonti}, {Tucker},
  {Uomoto}, {Vanden Berk}, {Vogeley}, {Waddell}, {Wang}, {Watanabe},
  {Weinberg}, {Yanny}, {Yasuda}, \& {SDSS Collaboration}}]{York00}
{York} D.~G., {Adelman} J., {Anderson} Jr. J.~E., {Anderson} S.~F., {Annis} J.,
  {Bahcall} N.~A., {Bakken} J.~A., {Barkhouser} R., {Bastian} S., {Berman} E.,
  {Boroski} W.~N., {Bracker} S., {Briegel} C., {Briggs} J.~W., {Brinkmann} J.,
  {Brunner} R., {Burles} S., {Carey} L., {Carr} M.~A., {Castander} F.~J.,
  {Chen} B., {Colestock} P.~L., {Connolly} A.~J., {Crocker} J.~H., {Csabai} I.,
  {Czarapata} P.~C., {Davis} J.~E., {Doi} M., {Dombeck} T., {Eisenstein} D.,
  {Ellman} N., {Elms} B.~R., {Evans} M.~L., {Fan} X., {Federwitz} G.~R.,
  {Fiscelli} L., {Friedman} S., {Frieman} J.~A., {Fukugita} M., {Gillespie} B.,
  {Gunn} J.~E., {Gurbani} V.~K., {de Haas} E., {Haldeman} M., {Harris} F.~H.,
  {Hayes} J., {Heckman} T.~M., {Hennessy} G.~S., {Hindsley} R.~B., {Holm} S.,
  {Holmgren} D.~J., {Huang} C.-h., {Hull} C., {Husby} D., {Ichikawa} S.-I.,
  {Ichikawa} T., {Ivezi{\'c}} {\v Z}., {Kent} S., {Kim} R.~S.~J., {Kinney} E.,
  {Klaene} M., {Kleinman} A.~N., {Kleinman} S., {Knapp} G.~R., {Korienek} J.,
  {Kron} R.~G., {Kunszt} P.~Z., {Lamb} D.~Q., {Lee} B., {Leger} R.~F.,
  {Limmongkol} S., {Lindenmeyer} C., {Long} D.~C., {Loomis} C., {Loveday} J.,
  {Lucinio} R., {Lupton} R.~H., {MacKinnon} B., {Mannery} E.~J., {Mantsch}
  P.~M., {Margon} B., {McGehee} P., {McKay} T.~A., {Meiksin} A., {Merelli} A.,
  {Monet} D.~G., {Munn} J.~A., {Narayanan} V.~K., {Nash} T., {Neilsen} E.,
  {Neswold} R., {Newberg} H.~J., {Nichol} R.~C., {Nicinski} T., {Nonino} M.,
  {Okada} N., {Okamura} S., {Ostriker} J.~P., {Owen} R., {Pauls} A.~G.,
  {Peoples} J., {Peterson} R.~L., {Petravick} D., {Pier} J.~R., {Pope} A.,
  {Pordes} R., {Prosapio} A., {Rechenmacher} R., {Quinn} T.~R., {Richards}
  G.~T., {Richmond} M.~W., {Rivetta} C.~H., {Rockosi} C.~M., {Ruthmansdorfer}
  K., {Sandford} D., {Schlegel} D.~J., {Schneider} D.~P., {Sekiguchi} M.,
  {Sergey} G., {Shimasaku} K., {Siegmund} W.~A., {Smee} S., {Smith} J.~A.,
  {Snedden} S., {Stone} R., {Stoughton} C., {Strauss} M.~A., {Stubbs} C.,
  {SubbaRao} M., {Szalay} A.~S., {Szapudi} I., {Szokoly} G.~P., {Thakar} A.~R.,
  {Tremonti} C., {Tucker} D.~L., {Uomoto} A., {Vanden Berk} D., {Vogeley}
  M.~S., {Waddell} P., {Wang} S.-i., {Watanabe} M., {Weinberg} D.~H., {Yanny}
  B., {Yasuda} N., {SDSS Collaboration}, 2000, \aj, 120, 1579

\end{thebibliography}

